Neutrino Mass and Proton Decay in a ${U(1)}_R$ Symmetric Model

We study a ${U(1)}_R$ symmetric extenstion of supersymmetric standard model with supersymmetry breaking in the visible as well as hidden sectors. Specifically we study ${U(1)}_R$ breaking effects parametrized by the gravitino mass. A special $R$-charge assignment of right-handed neutrinos allows us to have neutrino Yukawa couplings with the $R$-charged Higgs field, which develops a tiny vacuum expectation value after the inclusion of $U(1)_R$ symmetry breaking. Even with O(1) Yukawa couplings, a suitable size of Dirac neutrino masses can be generated if the gravitino mass is very small, $m_{3/2}=1\hbox{---}10\,\mathrm{eV}$. Our flipped $R$-charge assignment also allows a new type of dimension five operator that can induce the proton decay. It turns out that the proton stability mildly constrains the allowed range of the gravitino mass: Gravitino heavier than $10 \ \mathrm{keV}$ can evade the proton decay constraint as well as cosmological ones. In this case, the largest neutrino Yukawa coupling is comparable to the electron Yukawa. We also calculate the mass of the pseudo goldsino and its mixing to neutralinos, and briefly discuss its implications in cosmology and Higgs phenomenology.

==> macro_MNS.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%  Personal Macros (1) %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% correction line
\usepackage{ulem}  % \sout{ text }
\newcommand{\rsout}[1]{\textcolor{red}{\sout{#1}}} % \rsout{ text }
\newcommand{\bsout}[1]{\textcolor{blue}{\sout{#1}}} % \rsout{ text }
\newcommand{\rxout}[1]{\textcolor{red}{\xout{#1}}} % \rsout{ text }
\newcommand{\bxout}[1]{\textcolor{blue}{\xout{#1}}} % \rsout{ text }
\newcommand{\gxout}[1]{\textcolor{green}{\xout{#1}}} % \rsout{ text }

%%% color
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}
\definecolor{darkgreen}{rgb}{0, 0.5, 0.2}
\newcommand{\green}[1]{{\color{darkgreen} #1}}

\allowdisplaybreaks[4]
\newcommand{\lsim}{%
\raise0.3ex\hbox{$\;<$\kern-0.75em\raise-1.1ex\hbox{$\sim\;$}}}
\newcommand{\gsim}{%
\raise0.3ex\hbox{$\;>$\kern-0.75em\raise-1.1ex\hbox{$\sim\;$}}}
%\newcommand{\tr}{\mathrm{Tr}\,}
\newcommand{\Slash}[1]{\ooalign{\hfil{\bf $ \diagup $}\hfil\crcr$#1$}}
\renewcommand{\baselinestretch}{1.1}

\newcommand{\alt}{\lsim}
\newcommand{\agt}{\gsim}

% show label
%\usepackage{showkeys}

%%%%%%%\usepackage{array,arydshln}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%  Personal Macros (2) %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\non}{\nonumber}
\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\Eq}[1]{Eq.~(\ref{#1})}
\newcommand{\eqs}[2]{(\ref{#1})--(\ref{#2})}
\newcommand{\Eqs}[2]{Eqs.~(\ref{#1})--(\ref{#2})}
%%%%% equations
\newcommand{\ba}{\begin{eqnarray}}
\newcommand{\ea}{\end{eqnarray}}
\newcommand{\leftB}{\Bigl}
\newcommand{\rightB}{\Bigr}
%%% roman character
\newcommand{\ala}{{\it \`a la}\ }
%\newcommand{\ie}{{\it i}.{\it e}.}
\newcommand{\st}{{\it s}.{\it t}.}
%\newcommand{\eg}{{\it e}.{\it g}.}
\newcommand{\hc}{\mbox{H.c.}}       % in mathmode.

\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\wh}[1]{{\widehat #1}}
\newcommand{\wt}[1]{{\widetilde #1}}
\newcommand{\VEV}[1]{\left<#1\right>}
\newcommand{\order}[1]{\mathcal{O}\!\left(#1\right)}
\newcommand{\fun}[1]{\!\left(#1\right)} % fir arguments of a function

\newcommand{\units}[1]{\,\mathrm{[#1]}} % for units
\newcommand{\nunits}[1]{\,\mathrm{#1}}  % for numerical values with units

\newcommand{\wb}[1]{%
\vbox{\ialign{##\crcr\hskip 1.0pt\hrulefill\hskip 0.3pt%
\crcr\noalign{\kern-1pt\vskip0.07cm\nointerlineskip}%
$\hfil\displaystyle{#1}\hfil$\crcr}}}

\newcommand{\mxino}{m_{\wt{X}_0}}
\newcommand{\mbino}{m_{\wt{B}}}
\newcommand{\mwino}{m_{\wt{W}^3}}
\renewcommand{\mwino}{m_{\wt{W}}}

\newcommand{\matrixtwo}[4]{
\left(\begin{array}{cc} %
{#1} & {#2} \\ {#3} & {#4} %
\end{array}\right)%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%  \braket<#1|#2|#3> and \bracket{#1|#2|#3}  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\braket<#1|#2|#3>{%
\gdef\@bra{#1}\gdef\@opr{#2}\gdef\@ket{#3}\@braket}
\def\bracket#1{\expandafter\bunri#1\@nil\relax\@braket}
\def\bunri#1|#2|#3\@nil{%
\gdef\@bra{#1}\gdef\@opr{#2}\gdef\@ket{#3}}
\def\@braket{\setbox0=\hbox{$\displaystyle {\@bra}{\@ket}$}
	\dimen0\ht0 \dimen1\dp0
	\setbox0=\hbox{$\displaystyle {\@opr}$}
	\@tempdima=.8\ht0 \@tempdimb=.8\dp0
	\ifdim\@tempdima>\dimen0\relax\dimen0=\@tempdima\fi
	\ifdim\@tempdimb>\dimen1\relax\dimen1=\@tempdimb\fi
	\setbox1=\hbox{\vrule height\dimen0 depth\dimen1 width\z@}
	\def\Strut{\relax\ifmmode\copy1\else\unhcopy1\fi}
	\def\sp@ce{\kern.09em}
	\ifx\@bra\empty\relax
	 \ifx\@opr\empty\relax \left|\Strut\sp@ce{\@ket}\right>
	 \else 
	   \ifx\@ket\empty\relax \left<{\@opr}\right> 
	   \else {\@opr}\left|\Strut\sp@ce{\@ket}\right> \fi\fi
	\else
	 \ifx\@opr\empty\relax
	   \ifx\@ket\empty\relax \left<\Strut{\@bra}\sp@ce\right|
	   \else \left<\Strut{\@bra}\sp@ce\right|\left.
	                         \kern-.22em\Strut{\@ket}\right> \fi
	 \else 
	   \ifx\@ket\empty\relax\left<\Strut{\@bra}\sp@ce\right|{\@opr}
	   \else \left<\Strut{\@bra}\sp@ce\right|{\@opr}
	                \left|\Strut\sp@ce{\@ket}\right> \fi\fi\fi}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%  Personal Macros (3) %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mplanck}{M_{\mathrm{pl}}}           % for reduced planck

\newcommand{\LambdaC}{\Lambda_{\mathrm{cutoff}}} % cutoff for dim.5 op.
\newcommand{\LambdaD}{\Lambda_{\mathrm{D}}}      % cutoff for supersoft op.

\newcommand{\amp}{\mathrm{Amp}}
\renewcommand{\amp}{\mathcal{A}}

\newcommand{\cabbibo}{\varepsilon} 
\newcommand{\suppression}{\mathcal{Z}} % suppression factor of pG mass


\renewcommand{\paragraph}[1]{
\medskip\medskip
\noindent\underline{\hbox{\bf #1}}%${}$\\
}


